Improved Stability and Generalization Guarantees of the Decentralized SGD Algorithm

This paper presents a new generalization error analysis for Decentralized Stochastic Gradient Descent (D-SGD) based on algorithmic stability. The obtained results overhaul a series of recent works that suggested an increased instability due to decentralization and a detrimental impact of poorly-connected communication graphs on generalization. On the contrary, we show, for convex, strongly convex and non-convex functions, that D-SGD can always recover generalization bounds analogous to those of classical SGD, suggesting that the choice of graph does not matter. We then argue that this result is coming from a worst-case analysis, and we provide a refined optimization-dependent generalization bound for general convex functions. This new bound reveals that the choice of graph can in fact improve the worst-case bound in certain regimes, and that surprisingly, a poorly-connected graph can even be beneficial for generalization.

==> subfiles/macros.tex <==

% Definitions of handy macros can go here
\newcommand{\calD}{{\cal D}}
\newcommand\calX{{\cal X}}
\newcommand\calY{{\cal Y}}
\newcommand\calP{{\cal P}}
\newcommand\calE{{\cal E}}
\newcommand\calA{{\cal A}}
\newcommand\calS{{\cal S}}
\newcommand\calO{{\cal O}}
\newcommand\calR{{\cal R}}
\newcommand\calN{{\cal N}}
\newcommand\calZ{{\cal Z}}
\newcommand\calU{{\cal U}}


\newcommand\calRh{{\widehat{\cal R}}}
\newcommand\fh{{\widehat{f}}}
\newcommand\IE{{\mathbb{E}}}
\newcommand\IR{{\mathbb{R}}}
\newcommand\IN{{\mathbb{N}}}
\newcommand\IP{{\mathbb{P}}}
\newcommand\Chat{{\widehat{\mathcal{C}}}}
\newcommand\Qh{{\widehat{Q}}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\Ind}[1]{\mathbbm{1}\{#1\}}
\newcommand\be{{\boldsymbol{e}}}
\newcommand{\One}[1]{{\mathbbm{1}}\left\{{#1}\right\}}
\newcommand{\OneSm}[1]{{\mathbbm{1}}\{{#1}\}}
\newcommand{\Bin}{\mathrm{Bin}}
\newcommand{\PoisBin}{\mathrm{PoisBin}}




% COMMANDS, SHORTUCTS
\newcommand{\myemph}[1]{\textcolor{myblue}{#1}}
\newcommand{\myemphtwo}[1]{\textcolor{myorange}{#1}}
\newcommand{\myemphthree}[1]{\textcolor{mygreen}{#1}}
\newcommand{\ratio}{0.5}
\newcommand{\ratiob}{0.5}
\newcommand{\algo}{{\textsc{NurseNet}}\ }
\newcommand{\subalgo}{{\small\textsc{SPN}}\ }
\newcommand{\lghline}{\arrayrulecolor{lgray}\hline}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfz}{\mathbf{z}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfind}{\mathbf{1}}
\newcommand{\bbmind}{\mathbbm{1}}
%\newcommand\calX{\boldsymbol{\mathcal{X}}}
\newcommand{\iou}{\mathrm{IoU}}
\newcommand{\ie}            {i.e.\ }
\newcommand{\iid}           {i.i.d.\ }
\newcommand{\eg}            {e.g.\ }
\newcommand{\wrt}           {w.r.t.\ }
\newcommand{\cdf}           {c.d.f.\ }
\newcommand{\st}            {\mbox{s.t.\ }}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand\mymidrule{\specialrule{0.4pt}{1.5pt}{1.5pt}} % thiner midrule than original
\newcommand{\starw}{\ding{73}}%
\newcommand{\starb}{\ding{72}}%
\newcommand{\serr}{$\text{SER}_{\text{R}}$}
\newcommand{\serll}{$\text{SER}_{\text{LL}}$}
\newcommand{\strutnd}{$\text{STRUT}_{\text{IG}}$}
\newcommand{\struthi}{$\text{STRUT}_{\text{HI}}$}
\newcommand{\spm}{{\scriptsize $\pm$ }}  % smallesst +/- sign
\newcommand{\cRM}[1]{\MakeUppercase{\romannumeral #1}}  % chiffre romain Capital
\newcommand{\leaferr}{\varepsilon_{\text{leaf}}}  % leaf error
\newcommand{\sterr}{\varepsilon_{\text{subtree}}}  % subtree error
\newcommand{\IG}{\mathrm{IG}}
\newcommand{\DG}{\mathrm{DG}}
\newcommand{\JSD}{\mathrm{JSD}}
\newcommand{\KL}{\mathrm{KL}}
\newcommand{\TPR}{\mathrm{TPR}}
\newcommand{\TP}{\mathrm{TP}}
\newcommand{\FP}{\mathrm{FP}}
\newcommand{\TN}{\mathrm{TN}}
\newcommand{\FN}{\mathrm{FN}}
\newcommand{\FPR}{\mathrm{FPR}}
\newcommand{\Acc}{\mathrm{Accuracy}}
\newcommand{\AUC}{\mathrm{AUC}}
\newcommand{\RR}{\mathbb{R}} % espace réel
\newcommand{\XX}{\mathcal{X}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\EEE}[1]{\mathbb{E}_{#1}}

\newcommand{\TS}{\Tilde{S}}
\newcommand{\TW}{\widetilde{W}}
\newcommand{\TG}{\Tilde{G}}
\newcommand{\TZ}{\Tilde{Z}}
\newcommand{\Ttheta}{\Tilde{\theta}}
% \newcommand{\TS}{S'}
% \newcommand{\TG}{G'}
% \newcommand{\TZ}{Z'}
% \newcommand{\Ttheta}{{\theta'}}

\newcommand{\dbar}{\bar{\delta}}
\newcommand{\dsup}{\delta^{\sup}}

\newcommand{\supk}{\sup_{k\in\{1,\ldots,m\}}}
\newcommand{\supj}{\sup_{j\in\{1,\ldots,m\}}}



\newcommand{\PP}{\mathbb{P}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\calV}{\mathcal{V}}
%\newcommand{\calO}{\mathcal{O}}
%\newcommand{\calD}{\mathcal{D}}
%\newcommand{\calS}{\mathcal{S}}
\newcommand{\calF}{\mathcal{F}}

\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\1}{\mathbf{1}}

%\newcommand{\ratio}{0.31}%0.32
%\newcommand{\ratiob}{0.70}%0.81
%\newcommand{\ratiorwexp}{0.33}%0.32
\newcommand{\ratiorwexp}{0.49}%0.32


\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{assumption}{Assumption}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}

\newtheorem{lemma}{Lemma}






\setlength{\parindent}{0pt} 
\setlength{\parskip}{0.5em}

\newcommand{\textquote}[1] {\medskip
\hfill\begin{minipage}{0.95\textwidth}{``\textit{#1}''}\end{minipage}}

==> subfiles/old_proofs.tex <==

\begin{proposition}\label{prop:gen-avg-nonconv}
    Let $A(S)=\bar{\theta}^{(T)}$. Under the same set of hypotheses, the upper-bound derived in Theorem \ref{thme:non-convex} is also a valid upper-bound on $|\EE_{A,S}[R(A(S)) - R_S(A(S))]|$.
\end{proposition}

\begin{proof}


    We start by proving a result analogue to that Lemma \ref{lem:non-conv}. Let the event  $\mathcal{E}=\{\frac{1}{m}\sum_{k=1}^m\delta_k^{(t_0)}= 0\}$, using similar arguments, we have:

    \begin{align*}
        \EE_A[|\ell(\bar{\theta}^{(T)}; z) - \ell(\tilde{\bar{\theta}}^{(T)};z)|] & = \IP(\mathcal{E})\EE_A[|\ell(\bar{\theta}^{(T)}; z) - \ell(\tilde{\bar{\theta}}^{(T)};z)| \big| \mathcal{E}] +  \IP(\mathcal{E}^c)\EE_A[|\ell(\bar{\theta}^{(T)}; z) - \ell(\tilde{\bar{\theta}}^{(T)};z)| \big| \mathcal{E}^c] \\
        & \leq \EE_A[|\ell(\bar{\theta}^{(T)}; z) - \ell(\tilde{\bar{\theta}}^{(T)};z)| \big| \mathcal{E}] +\IP(\mathcal{E}^c)\cdot \sup_{\theta,z}\ell(\theta;z) \\ 
        & \leq L\EE_A[\|\bar{\theta}^{(t)}  - \tilde{\bar{\theta}}^{(t)}\| \big| \mathcal{E}]+\frac{t_0}{n} \\
        & \leq \frac{L}{m}\sum_{k=1}^m\EE_A[\|\theta_k^{(t)}  - \tilde{\theta}_k^{(t)}\| \big| \mathcal{E}]+\frac{t_0}{n}
    \end{align*}

We end up with a result analogous to Equation \eqref{eq:right-hand}. The rest of the proof is identical, taking $\Delta_t \triangleq \frac{1}{m}\sum_{k=1}^m\EE[\delta_k^{(t)} | \sum_{k}\delta_k^{(t_0)} = 0]$ and noticing that $\Delta_{t_0}=0$.
    
\end{proof}

% Our analysis for the non-convex case leverages the fact that D-SGD can make
% several steps before using the one example that has been swapped. This idea is
% summarized by the following lemma.

% \begin{lemma} \label{lem:non-conv} Assume that the loss function $\ell
% (\cdot,z)$ is nonnegative and $L$-Lipschitz for all $z$. Let $S$ and $S'$ be two samples of size $(m,n)$ differing in only a single example. Let $\theta_k^{(T)}$ and $\tilde{\theta}_k^{(T)}$ the outputs of agent $k = 1,\ldots, m$, after $T$ steps of D-SGD (Variant A and B) on $S$ and $S'$ respectively. Then, for every $z \in \calZ$ and every $t_0 \in \{0, 1, \ldots, T\}$ we have:
%     \begin{equation}
%         \EE_A[|\ell(\theta_k^{(T)}; z) - \ell(\tilde{\theta}_k^{(T)};z)|] \leq \frac{t_0}{n}\sup_{\theta, z} \ell(\theta;z) + L\EE[\delta_k^{(T)} | \delta_k^{(t_0)}= 0],
%     \end{equation}
%     where $\delta_k^{(t)} = \|\theta_k^{(t)}  - \tilde{\theta}_k^{(t)} \|$.
% \end{lemma}

% \begin{proof}
%     The proof is essentially the same as the one for Lemma 3.11 in \citet{hardt2016train}. It is detailed here for completeness. Let the event $\mathcal{E}=\{\delta_k^{(t_0)}= 0\}$, we have:

%     \begin{align*}
%         \EE_A[|\ell(\theta_k^{(T)}; z) - \ell(\tilde{\theta}_k^{(T)};z)|] & = \IP(\mathcal{E})\EE_A[|\ell(\theta_k^{(T)}; z) - \ell(\tilde{\theta}_k^{(T)};z)| \big| \mathcal{E}] +  \IP(\mathcal{E}^c)\EE_A[|\ell(\theta_k^{(T)}; z) - \ell(\tilde{\theta}_k^{(T)};z)| \big| \mathcal{E}^c] \\
%         & \leq \EE_A[|\ell(\theta_k^{(T)}; z) - \ell(\tilde{\theta}_k^{(T)};z)| \big| \mathcal{E}] +\IP(\mathcal{E}^c)\cdot \sup_{\theta,z}\ell(\theta;z) \\ 
%         & \leq L\EE_A[\|\theta_k^{(T)}  - \tilde{\theta}_k^{(T)}\| \big| \mathcal{E}]+\IP(\mathcal{E}^c)\cdot \sup_{\theta,z}\ell(\theta;z)
%     \end{align*}

%     It remains to bound $\IP(\mathcal{E}^c)$. Let $T_0$ be the random variable of the first time step D-SGD uses the swapped example. Then, we have $\{T_0 > t_0\} \subset \mathcal{E} \Leftrightarrow \mathcal{E}^c \subset \{T_0 \leq t_0\}$ and therefore $\IP(\mathcal{E}^c) \leq \IP(T_0 \leq t_0) = \sum_{t=1}^{t_0}\IP(T_0=t)\leq \frac{t_0}{n}$. This completes the proof.
    
% \end{proof}




% % \begin{lemma} \label{lem:non-conv} Assume that the loss function $\ell
% % (\cdot,z)$ is nonnegative and $L$-Lipschitz for all $z$. Let $S$ and $S'$ be two samples of size $(n,m)$ differing in only a single example. Denote by $\bar{\theta}^{(T)}=\frac{1}{m}\sum_{k=1}^m\theta_k^{(T)}$ and $\bar{\tilde{\theta}}^{(T)}=\frac{1}{m}\sum_{k=1}^m\tilde{\theta}_k^{(T)}$ the output of D-SGD after $T$ steps on $S$ and $S'$ respectively. Then, for every $z \in \calZ$ and every $t_0 \in \{0, 1, \ldots, T\}$ we have:
% %     \begin{equation}
% %         \EE_A[|\ell(\bar{\theta}^{(T)}; z) - \ell(\bar{\tilde{\theta}}^{(T)};z)|] \leq \frac{t_0}{n}\sup_{\theta, z} \ell(\theta;z) + L\EE[\dbar_T | \dbar_{t_0}= 0],
% %     \end{equation}
% %     where $\dbar_t = \frac{1}{m}\sum_{k=1}^m \|\theta_k^{(t)}  - \tilde{\theta}_k^{(t)} \|$.
% % \end{lemma}

% % \begin{proof}
% %     The proof is essentially the same as the one for Lemma 3.11 in \citet{hardt2016train}, with an additional use of triangular inequality to bound $\|\bar{\theta}^{(T)} - \bar{\tilde{\theta}}^{(T)}\|$ by $\dbar_T$.
% % \end{proof}

% We can now move on to the proof of the main theorem. We first apply Lemma \ref{lem:non-conv} and the fact that, by assumption, $\ell \in [0,1]$, so that for any $t_0 \in \{0, 1, \ldots, T\}$ and any $k=1,\ldots, m$, we have:
% \begin{equation}
%     \EE_A[|\ell(\theta_k^{(T)}; z) - \ell(\tilde{\theta}_k^{(T)};z)|] \leq \frac{t_0}{n} + L\EE[\delta_k^{(T)} | \delta_k^{(t_0)}= 0].
% \end{equation}

% Since this is true for all $z$ and neighboring datasets $S$ and $S'$, we can use a uniform stability argument (Lemma \ref{lemma:uniform_stab}) and get:

% \begin{equation}
% \label{eq:right-hand}
%     \frac{1}{m}\sum_{k=1}^m|\EE_{A,S}[R(A_k(S)) - R_S(A_k(S))]| \leq \frac{t_0}{n} + \frac{L}{m}\sum_{k=1}^m\EE[\delta_k^{(T)} | \delta_k^{(t_0)}= 0].
% \end{equation}

% It remains to control the right-hand term of Equation \eqref{eq:right-hand}. We start with the proof for the variant A of D-SGD. The proof for Variant B will follow.

% \textbf{Variant A:}

% The proof is analogous to the one obtained for convex cases 
% (Theorem \ref{thme:convex} and \ref{thme:strongly}) and we can start directly from Equation \eqref{eq:almost_sure_convex} using the same arguments.
    


%     Thanks to Lemma \ref{lem:expansivity} (part. 3), we notice that for all
%     $k$, the update rules $G_{\eta_t,Z_{I^t_kk}}(\theta)=\theta -\frac{\eta_t}{W_{kk}}\nabla\ell
%     (\theta;Z_{I^t_kk})$ and $G_{\eta_t,Z'_{I^t_kk}}(\theta)=\theta
%     -\frac{\eta_t}{W_{kk}}\nabla\ell(\theta;Z'_{I^t_kk})$ are $(1+\frac{\eta_t\beta}
%     {W_{kk}})$-expansive. Assume without loss of generality that the swapped sample is the $i$-th of the $j$-th agent. Then, following the proof of the convex cases, we can now split the analysis similarly.

%     \fbox{If $k \neq j$,} we have $Z_{I^t_kk} = Z'_{I^t_kk}$, which gives from Eq. \eqref{eq:almost_sure_convex} and Lemma \ref{lem:growth} with the $(1+\frac{\eta_t\beta}
%     {W_{kk}})$-expansivity, that:
%     \begin{align}
%         \|\theta_k^{(t+1)} - \tilde{\theta}_k^{(t+1)}\|_2  & \leq W_{kk} \Big(1+\frac{\eta_t\beta}
%     {W_{kk}}\Big)\Big\|\theta_k^{(t)}-\tilde{\theta}_k^{(t)}  \Big\|_2 + \sum^m_{l\neq j }W_{kl}\Big\|\theta_l^{(t)}-\tilde{\theta}_l^{(t)}  \Big\|_2 \nonumber \\
%     & = \sum^m_{l=1 }W_{kl}\Big\|\theta_l^{(t)}-\tilde{\theta}_l^{(t)}  \Big\|_2
%     + \eta_t\beta\Big\|\theta_k^{(t)}-\tilde{\theta}_k^{(t)}  \Big\|_2
%         \label{eq:recurs_k_nonconv}
%     \end{align}


% \fbox{If $k = j$:} \\

% \underline{With probability $1-\frac{1}{n}$}, $I^t_j\neq i$ so $Z_{I^t_jj} = Z'_{I^t_jj}$ and we therefore have again the relation of Eq. \eqref{eq:recurs_k_nonconv}.


% \underline{With probability $\frac{1}{n}$} however, $I^t_j=i$ and in that case $Z_{I^t_jj} = Z_{ij}\neq \TZ_{ij} =  Z'_{I^t_jj} $. 
% With probability $\frac{1}{n}$, we therefore have: 

% \begin{align}
%     \|\theta_j^{(t+1)} - \tilde{\theta}_j^{(t+1)}\|_2  & \leq W_{jj}\Big\|\theta_j^{(t)}- \frac{\eta_t}{W_{jj}}\nabla \ell(\theta^{(t)}_j;Z_{ij}) - \tilde{\theta}_j^{(t)} + \frac{\eta_t}{W_{jj}}\nabla \ell(\tilde{\theta}^{(t)}_j;\title{Z}_{ij})\Big\|_2 + \sum^m_{l\neq j}W_{jl}\Big\|\theta_l^{(t)}-\tilde{\theta}_l^{(t)}  \Big\|_2 \nonumber  \\
%     & \hspace{-0.2cm} \overset{Lem. \ref{lem:growth}}{\leq}  \hspace{-0.2cm} W_{jj}\Big(\big(1+\frac{\eta_t\beta}
%     {W_{kk}}\big)\|\theta_j^{(t)}-\tilde{\theta}^{(t)}_j\|_2 + \frac{2\eta_t L}{W_{jj}}\Big)+ \sum^m_{l\neq j}W_{jl}\Big\|\theta_l^{(t)}-\tilde{\theta}_l^{(t)}  \Big\|_2 \nonumber  \\
%     & = \sum^m_{l=1}W_{jl}\Big\|\theta_l^{(t)}-\tilde{\theta}_l^{(t)}  \Big\|_2 + \eta_t\beta\Big\|\theta_j^{(t)}-\tilde{\theta}_j^{(t)}  \Big\|_2 + 2\eta_t L \nonumber
% \end{align}

% Let $\Delta_t \triangleq \frac{1}{m}\sum_{k=1}^m\EE[\delta_k^{(t)} | \delta_k^{(t_0)} = 0]$. Then, from the previous equations, using the double stochasticity of $W$ and the fact that $\eta_t\leq \frac{c}{t+1}$, $c>0$, we have $\forall t\geq t_0$:
% \begin{align}
%     \Delta_{t+1} & \leq (1+\eta_t\beta)\Delta_{t} + \frac{2\eta_t L}{mn} \nonumber \\
%     & \leq \Big(1+\frac{c\beta}{t+1}\Big)\Delta_{t} + \frac{2cL}{(t+1)mn} \nonumber \\
%     & \leq \exp{\Big(\frac{c\beta}{t+1}\Big)}\Delta_{t}+ \frac{2cL}{(t+1)mn}\;,
%     \label{eq:start-variant-B}
% \end{align}

% where the last inequality uses the fact that $1+x\leq \exp(x)$. Now, since $\Delta_{t_0} = 0$, we can unroll the recursion from $T$ to $t_0+1$ and get:
% \begin{align}
%     \Delta_T & \leq \frac{2cL}{Tmn} + \sum_{t=t_0+1}^{T-1}\Big\{\prod_{k=t+1}^T \exp \Big(\frac{c\beta}{k}\Big)\Big\}\frac{2cL}{tmn} \nonumber \\ 
%     & = \frac{2cL}{Tmn} + \sum_{t=t_0+1}^{T-1}\exp \Big(c\beta\sum_{k=t+1}^T \frac{1}{k}\Big)\frac{2cL}{tmn} \nonumber \\
%     & \leq \frac{2cL}{Tmn} + \sum_{t=t_0+1}^{T-1}\exp \Big(c\beta \log\big(\frac{T}{t}\big)\Big)\frac{2cL}{tmn} \nonumber \\
%     & = \frac{2cL}{Tmn} + \sum_{t=t_0+1}^{T-1}\Big(\frac{T}{t}\Big)^{c\beta}\frac{2cL}{tmn}\nonumber \\
%     & = \frac{2cLT^{c\beta}}{T^{c\beta +1}mn} + \frac{2cLT^{c\beta}}{mn}\sum_{t=t_0+1}^{T-1} t^{-c\beta-1} \nonumber \\
%     & = \frac{2cLT^{c\beta}}{mn}\sum_{t=t_0+1}^{T} t^{-c\beta-1} \nonumber \\
%     & \leq \frac{2cLT^{c\beta}}{mn} \frac{t_0^{-\beta c}}{c\beta} = \frac{2L}{\beta mn}\Big(\frac{T}{t_0}\Big)^{c \beta}, \label{eq:recursion-non-convex}
% \end{align}
% where the last inequality is obtained using bounds over (partial) harmonic series. 


% Plugging this result into \eqref{eq:right-hand}, we obtain
% \begin{equation*}
%     \frac{1}{m}\sum_{k=1}^m|\EE_{A,S}[R(A_k(S)) - R_S(A_k(S))]| \leq \frac{t_0}{n} + \frac{2L^2}{\beta mn}\Big(\frac{T}{t_0}\Big)^{c \beta}.
% \end{equation*}

% Then, taking $t_0 = \Big(\frac{2L^2c}{m}\Big)^{\frac{1}{c\beta + 1}}T^{\frac{c\beta}{c\beta + 1}}$ (minimizer of the right-hand term above), we have 
% \begin{equation*}
%     \frac{1}{m}\sum_{k=1}^m|\EE_{A,S}[R(A_k(S)) - R_S(A_k(S))]| \leq (1+\frac{1}{\beta c})(2cL^2)^{\frac{1}{\beta c +1}}\frac{T^{\frac{\beta c}{\beta c +1}}}{m^{\frac{1}{\beta c +1}}n}\;,
% \end{equation*}
% which concludes the proof for Variant A.

% \textbf{Variant B:}

% The proof for the variant B is essentially the same, where instead of Equation \eqref{eq:almost_sure_convex}, we have:

%     \begin{align}
%         \|\theta_k^{(t+1)} -  \tilde{\theta}_k^{(t+1)}\|_2  & = \Big\|\sum^m_{l=1}W_{kl}\Big(\theta_l^{(t)} - \eta_t\nabla \ell(\theta^{(t)}_l;Z_{I^t_ll})\Big) - \sum^m_{l=1}W_{kl}\Big(\tilde{\theta}_l^{(t)} + \eta_t\nabla \ell(\tilde{\theta}^{(t)}_l;Z'_{I^t_ll})\Big)\Big\|_2 \nonumber  \\
%         & = \sum^m_{l=1}W_{kl}\Big\|\theta_l^{(t)} - \eta_t\nabla \ell(\theta^{(t)}_l;Z_{I^t_ll}) + \tilde{\theta}_l^{(t)} + \eta_t\nabla \ell(\tilde{\theta}^{(t)}_l;Z'_{I^t_ll})\Big\|_2
%         \label{eq:almost_sure-nonconvex}
%     \end{align}

% Since, thanks to Lemma \ref{lem:expansivity} (part. 1), the update rules $G_{\eta_t,Z_{I^t_ll}}(\theta)=\theta -\eta_t\nabla\ell(\theta;Z_{I^t_ll})$ and $G_{\eta_t,Z'_{I^t_ll}}(\theta)=\theta -\eta_t\nabla\ell(\theta;Z'_{I^t_ll})$ are $(1+\eta_t\beta)$-expansive, we can use the same arguments as before to show that

% \begin{equation*}
%     \EE[\|\theta_l^{(t)} - \eta_t\nabla \ell(\theta^{(t)}_l;Z_{I^t_ll}) + \tilde{\theta}_l^{(t)} + \eta_t\nabla \ell(\tilde{\theta}^{(t)}_l;Z'_{I^t_ll})\|\mathcal{F}_t] \leq (1+\eta_t\beta)\|\theta_l^{(t)} - \tilde{\theta}_l^{(t)}\| + \frac{2L\eta_t}{n}\mathds{1}_{\{l=j\}}
% \end{equation*}

% Combining this last equation with Eq. \eqref{eq:almost_sure-nonconvex} and using the double stochasticity of $W$ allows to recover the relation $\Delta_{t+1} \leq (1+\eta_t\beta)\Delta_{t} + \frac{2\eta_t L}{mn} $. From this point, the proof is the same as the one of Variant A, starting from the derivation of Equation \eqref{eq:start-variant-B}.

% \hfill\qedsymbol{}


==> subfiles/on-average.tex <==
%% !TEX root = ../neurips_2023.tex

\section{On-average generalization error}
\label{sec:on-svg}



This section presents our first main contribution. Following prior work 
\citep{sun2021stability,zhu2022topology,taheri2023generalization}, we prove
generalization bounds for the \emph{average of final iterates} $\bar{\theta}^{(T)}=\frac{1}{m}\sum_
{j=1}^m\theta_j^{(T)}$ of D-SGD.\footnote{Considering the average of final
iterates is also common when analyzing the optimization error of D-SGD, see
for instance \citep{koloskova2020unified,ying2021exponential}}
Our bounds contradict
(and improve upon) the recent results of \citet{sun2021stability}, who claimed
that the generalization error of D-SGD was badly impacted by sparse
communication graphs and obtained vacuous bounds for non-connected
 graphs. Remarkably, our results demonstrate that the generalization error of
 D-SGD is in fact \emph{not} impacted by the choice of communication graph,
 or by decentralization at all, as
 we essentially recover the bounds proved by \citet{hardt2016train} for
 \emph{centralized} SGD.

Throughout this section, we define $A(S)=
\bar{\theta}^{(T)}$.

%\aurelien{note: si besoin de gagner de la place, on pourrait mettre certains
%cas en appendix et simplement donner les messages principaux}

% This section presents our first main contribution. Following the analysis of \citet{hardt2016train} made for the (centralized) SGD algorithm, we demonstrate that the generalization error of D-SGD is not impacted by decentralization when $A(S)$ corresponds the \emph{average of final iterates}. Indeed, because of the decentralized nature of D-SGD, $m$ different parameters (one per agent) are learned at the final iterate $T$, denoted by $\theta_1^{(T)},\ldots,\theta_m^{(T)}$. For this reason, state-of-the-art theoretical analyses, whether it is regarding the optimization error \citep{koloskova2020unified,ying2021exponential} or the generalization error \citep{sun2021stability,zhu2022topology,taheri2023generalization}, rely instead on the average of final iterates $A(S)=\bar{\theta}^{(T)}=\frac{1}{m}\sum_{j=1}^m\theta_j^{(T)}$.

% The following generalization analysis contradicts (and improves upon) the
% recent results of \citet{sun2021stability}, who claimed that the generalization
%  error of the averaged final iterates was badly impacted by sparse communication graphs, and even vacuous for non-connected topologies. %In the following, we give generalization

\subsection{Convex loss functions}


\begin{theorem} \label{thme:convex}
    Assume that the loss function $\ell(\cdot;z)$ is convex, $L$-lipschitz (Assumption \ref{ass:lipschitz}) and $\beta$-smooth (Assumption \ref{ass:smooth}). Let $A(S)$ be the average of final iterates of D-SGD run for $T$ iterations and with $\eta_t\leq 2/\beta$. Then, D-SGD has a bounded expected generalization error:

    \begin{equation}
        |\EE_{A,S}[R(A(S)) - R_S(A(S))]| \leq \frac{2L^2 \sum_{t=0}^
        {T-1}\eta_t}{mn}\;.
    \end{equation}
\end{theorem}

% 
%\aurelien{pourquoi ces tildes plutôt que des $'$ comme pour les datasets?}

% \aurelien{aussi, jusqu'à maintenant l'index des agents était $j$, maintenant on utilise $k$}

%\aurelien{also in this sketch (or after in the discussion), I would explain
% that prior results are suboptimal because they mimic the optimization
% error analysis by controlling the consensus distance, while we take a
% different (and simpler) route.}
\begin{proof}[Sketch of proof (see Appendix \ref{app:convex} for details)] 

    Prior results \citep{sun2021stability,taheri2023generalization} are
    suboptimal because they try to mimic state-of-the-art \emph{optimization
    error} analyses \citep{kong2021consensus} which require to control a 
    \emph{consensus distance} term $\sum_k\|\theta^{(t)}_k - \bar{\theta}^{(t)}\|$. This term, important to ensure the minimization of the empirical risk, is small when all local parameters are close to each other, which is the case only if the communication graph is sufficiently connected. In the following proof, we provide a tighter (and simpler) analysis, which does not require the control of such consensus distance term.

    Denote by $\bar{\theta}^{(T)}=\frac{1}{m}\sum_{k=1}^m\theta_k^{(T)}$, and  $\bar{\Ttheta}^{(T)}=\frac{1}{m}\sum_{k=1}^m\Ttheta_k^{(T)}$, the average of final iterates for D-SGD run over two data sets $S$ and $S'$ that differ in only one sample. Noticing that ${\|\bar{\theta}^{(t+1)} - \bar{\Ttheta}^{(t+1)}\|}_2  \leq \bar{\delta}_{t+1} \triangleq \frac{1}{m}\sum_{k=1}^m {\|\theta_k^{(t+1)}  - \Ttheta_k^{(t+1)} \|}_2 $, the objective of the proof is to find a recurrence relation over the iterates of $\EE[\dbar_t]$ in order to prove that $\EE[\dbar_T]\leq   \frac{2L \sum_{t=0}^{T-1}\eta_t}{mn}$ and finally use Lemma \ref{lemma:ob-avg-gen} to conclude the proof.

    Using triangle inequalities and the double stochasticity of $W$ 
    (Assumption \ref{ass:doubly}), we show that $\dbar_{t+1} \leq \frac{1}{m} \sum^m_{k=1}\|G^{(t)}_k(\theta_k^{(t)}) -  \TG^{(t)}_k(\Ttheta_k^{(t)})\|_2$, where $G^{(t)}_k$ (respectively $\TG^{(t)}_k$) is the standard stochastic gradient update rule (Def. \ref{def:sgd-update-rule} in Appendix \ref{app:lemmas}) of agent $k$ at time $t$, computed over data set $S$ (respectively $S'$). Importantly, these update rules do not depend on $W$. Moreover, since only one sample is different between $S$ ans $S'$, only one agent has different update rules.

    At this point of the proof, we are in a scheme similar to that of 
    \citet{hardt2016train} who proposes different results to bound the
    difference $\|G^{(t)}_k(\theta_k^{(t)}) -  \TG^{(t)}_k(
    \Ttheta_k^{(t)})\|_2$ (Appendix \ref{app:lemmas}). Thanks to them,
    we show that with probability $1-\frac{1}{n}$, $\dbar_{t+1}\leq \dbar_t$, and with probability $\frac{1}{n}$, $\dbar_{t+1}\leq \dbar_t + \frac{2L\eta_t}{m}$. Using the fact that $\dbar_0 = 0$, it follows that: $$\EE[\dbar_T]\leq \EE[\dbar_T] + \frac{2L\eta_t}{mn} \leq \ldots \leq 0 + \frac{2L \sum_{t=0}^{T-1}\eta_t}{mn}\;,$$
    which concludes the proof.
\end{proof}

%\bat{Prior results \citep{sun2021stability,taheri2023generalization} are suboptimal because they try to mimic state-of-the-art \emph{optimization error} analyses \citep{kong2021consensus}, where appears a \emph{consensus distance} term $\sum_k\|\theta^{(t)}_k - \bar{\theta}^{(t)}\|$. This term, important to ensure the minimization of the empirical risk, is small only when all local parameters are close to each other, which is the case only if the communication graph is sufficiently connected. In the following proof, we provide a tighter (and even simpler) analysis, which does not require the control of such consensus distance term.}

    Theorem \ref{thme:convex} % is proved in detail in Appendix 
    % \ref{app:convex}. Its result
    shows that for convex functions, we recover the exact same generalization
    bound for D-SGD as the one obtained by \citet{hardt2016train} for
    centralized SGD, a result known to be optimal \citep{zhang2022stability}.
    This contradicts the recent results of \citet{sun2021stability}, who
    obtained bounds of order $\calO(\frac{T}{mn}+\frac{1}{\rho})$ for D-SGD,
    where $\rho \in [0,1]$ is the spectral gap of $W$. This former result was
    therefore claiming that the generalization error is strongly impacted by
    the connectivity of $W$ (tending to infinity as the graph becomes sparser), which is in fact not true as demonstrated by our
    result. Strikingly, their bound is not even consistent in the
    sense that it does not tend to $0$ as $n$ grows.

    The fact that our generalization bound for D-SGD matches the one of
    centralized SGD may seem surprising at first, but it simply comes
    from considering the average final iterate $\bar{\theta}^{(T)}=
    \frac{1}{m}\sum_{j=1}^m\theta_j^{(T)}$. Indeed,
    this makes the algorithm more stable,
    erasing
    the impact of the communication graph $W$ in a somewhat artificial way 
    (since a global averaging step is incompatible with the decentralized
    scenario). In Section~\ref{sec:worst-case}, we will introduce what we
    think is a more suitable notion of generalization error for D-SGD, and
    show that this quantity does depend on the choice of communication
    graph.
    % We will
    % see later how we can make the impact of
    % the communication
    % graph appear in the generalization bound, by looking at another quantity than the final iterates averaging.

    %\bat{Batiste: Ajouter une explications de pourquoi les preuves des gars precedents ne fonctionnaient pas ?}



\subsection{Strongly convex loss functions}

We now consider strongly convex functions. As such functions cannot be
Lipschitz (Assumption \ref{ass:lipschitz}) over $\IR^d$, we restrict our
analysis to the optimization over a convex compact set $\Theta$ as done by
\citet{hardt2016train}. Denoting by $\Pi_\Theta(\Ttheta) = \argmin_{\theta \in \Theta}\|
\Ttheta - \theta\|$ the Euclidean projection onto $\Theta$, we consider the
\emph{projected} extension of the D-SGD algorithm, which replaces the
stochastic gradient update step from Algorithm~\ref{alg:d-sgd} by:
\begin{equation*}
    \theta_j^{(t + \frac{1}{2})} \gets \Pi_\Theta\Big(\theta_j^{(t)} -
    \eta_t\nabla \ell(\theta^{(t)}_j;Z_{I^t_jj})\Big)\;.
\end{equation*}

Before moving to our generalization result, we note that this algorithm is
well-suited to solving Tikhonov regularization problems, which
makes it quite natural to consider in practice.

\begin{theorem} \label{thme:strongly} Assume that the loss function $\ell
(\cdot;z)$ is $\mu$-strongly convex, $L$-Lipschitz over $\Theta$
(Assumption~\ref{ass:lipschitz}) and $\beta$-smooth (Assumption~\ref{ass:smooth}). Let $A(S)$ be the average of final iterates of the projected D-SGD run for $T$ iterations and with constant stepsize $\eta\leq 1/\beta$. Then, (projected) D-SGD has a bounded expected generalization error:
    \begin{equation}
        |\EE_{A,S}[R(A(S)) - R_S(A(S))]| \leq \frac{4L^2}{\mu mn}\;.
    \end{equation} 
    
\end{theorem}



    The proof of Theorem \ref{thme:strongly}, provided in Appendix 
    \ref{app:strongly-convex}, essentially follows the same scheme as the one
    derived above for convex functions. Once again, the bound matches the
    optimal one obtained for centralized SGD with strongly convex functions in
    \citet{hardt2016train}.
    Note that contrary to the general convex case, the generalization bound for strongly convex functions is independent of the number of iterations $T$, which makes these problems more stable and less likely to overfit.


    In the work of \citet{sun2021stability}, the authors have an additional
    error term in $\calO(\frac{1}{\mu\rho})$. Their generalization
    bound is therefore \emph{not} tending to $0$ as the number of samples
    increases and is vacuous when the communication graph is not connected ($\rho=0$). This again illustrates the suboptimality of these previous results and the major gain brought by ours.


\subsection{Non-convex loss functions}

Hereafter we provide a generalization error bound for \emph{bounded} non-convex functions. The proof is deferred to Appendix \ref{app:non-convex}.

\begin{theorem}
    \label{thme:non-convex}
    Assume that $\ell(\cdot;z) \in [0,1]$ is an $L$-Lipschitz
    (Assumption~\ref{ass:lipschitz}) and $\beta$-smooth
    (Assumption~\ref{ass:smooth}) loss function for every $z$. Let $A(S)$ be
    the average of final iterates of D-SGD run for $T$ iterations and with monotonically non-increasing step sizes $\eta_t\leq \frac{c}{t+1}$, $c>0$. Then, D-SGD has a bounded expected generalization error:
    \begin{equation}
        |\EE_{A,S}[R(A(S)) - R_S(A(S))]| \leq (1+\frac{1}{\beta c})(2cL^2)^{
        \frac{1}{\beta c +1}}\frac{T^{\frac{\beta c}{\beta c +1}}}{m^{\frac{1}{\beta c +1}}n}\;.
    \end{equation}
\end{theorem}

When omitting constant factors in $\beta$, $c$ and $L$, the non-convex
generalization bound becomes of order $\calO(T^{\frac{\beta c}{\beta c
+1}}/nm^{\frac{1}{\beta c +1}})$. Several comments are in order. First,
contrary to the convex cases, our bound does not exactly match the one of 
\citet{hardt2016train}. Indeed, when centralized SGD is run over $mn$ data
points, \citet{hardt2016train} obtain a bound of order $\calO(T^{\frac{\beta
c}{\beta c +1}}/nm)$ which is strictly better than our bound. This comes from
the fact that the proof technique relies on characterizing the number of steps
that occur before the algorithm picks the data point that differs in $S$ and
$S'$. In centralized SGD, the probability to pick this
point is $1/mn$ at each iteration, while it is only $1/n$ for D-SGD.
Importantly, this means that the weaker bound is not directly due to
decentralization, but rather to the fact that D-SGD selects $m$ samples at
each iteration (instead of only one for SGD). A fairer comparison would
thus be to compare D-SGD to centralized SGD with batch size $m$.

On a more positive note, our generalization bound is still independent of the
choice of graph and is tending towards $0$ as $n$ and $m$ increase. This
significantly improves the results obtained for
D-SGD in prior work, notably the one of \citet{sun2021stability}, who obtained
a bound of order $\calO(T^{\frac{\beta c}{\beta c +1}}(1/nm + C_\rho))$, where
$C_\rho$ tends to infinity as the spectral gap $\rho$ of $W$ tends to $0$ 
(e.g., as the communication graph gets sparser or as $m$ goes to infinity).

% \marc{J'aime pas trop la remarque ici qui plante un peu et qui dirait alors pourquoi vous ne l'avez pas fait si c'est facile? On peut la tourner plus positivement et la mettre encore en future work. Du genre
%  It has been recently proved \citep{zhang2022stability} that the proof of \citet{hardt2016train} is not  tight. The proof techniques in \citet{zhang2022stability} do not impact the reasoning here and our conclusions are essentially the same regarding the impact of the communication graph.}
\begin{remark}
    It has been recently shown \citep{zhang2022stability} that the proof of 
    \citet{hardt2016train} is not tight in all regimes. However, using the
    refined proof techniques from \citet{zhang2022stability} would not impact
    our main conclusions regarding the impact of the communication graph.

\end{remark}

%\bat{PL non convex loss ?}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../neurips_2023"
%%% End:


==> subfiles/supremum.tex <==
% !TEX root = ../neurips_2023.tex

\section{From on-average to worst-case generalization error}
\label{sec:worst-case}

In the previous section, we saw that if we consider the output of D-SGD to be
the average of the $m$ final iterates, the generalization error is not impacted by decentralization.
% In convex cases, the obtained bounds are even the same as those obtained for classical SGD.
Nevertheless, this implicitly assumes that a global averaging step is
performed at the end of the algorithm, which is not compatible
with the constraints of decentralization and would be very costly when the
number of agents is large.
% it appears that this full final
% averaging step is not very realistic in the decentralized setting, especially if the number of agents is high.
%\sugaurelien{In fact, this averaging step is often used to simplify the
%theoretical analysis of the optimization error, but does not take part of the D-SGD algorithm in practice.}{}

%\aurelien{de nouveau on utilise $k$ plutôt que $j$ pour l'index des agents}

In this section, we propose a new notion of generalization error that
is better-suited to decentralized algorithms, which output $m$ different
 models (one per agent). To this aim, we denote by $A_1(S),\ldots,A_m(S)$ the $m$ different outputs generated by a decentralized algorithm $A$ and we propose to control the \emph{worst-case expected generalization error given by} %the following definition.
\begin{equation}
\supj|\EE_{A,S}[R(A_j(S)) - R_S(A_j(S))]|\;.
\end{equation}

Similarly to classical analyses, we can propose a new notion of stability adapted to the decentralized framework and sufficient to control the above worst-case generalization error.

\begin{definition}\emph{(Worst-model stability).} \label{def:worst-stable} Consider the notations of Def. \ref{def:on-average}. A decentralized algorithm $A$ with $m$ outputs is said worst-model $\varepsilon$-stable if
    \begin{equation}
        \EE_{S,\TS,A}\Big[\frac{1}{mn}\sum_{i=1}^n\sum_{j=1}^m \supk \|A_k(S) - A_k(S^{(ij)})\|_2\Big] \leq \varepsilon \;.
    \end{equation}
    
\end{definition}

\begin{lemma}\emph{(Worst-case generalization via worst-model stability).} 
\label{lemma:ob-sup-gen} Let $A$ be worst-model $\varepsilon$-stable. Then, under Assumption~\ref{ass:lipschitz}, $\supj|\EE_{A,S}[R(A_j(S)) - R_S(A_j(S))]| \leq L \varepsilon$.
    
\end{lemma}

This lemma is a key element of our analysis as it states that it is sufficient
to control the worst-model stability in order to control the wors-case generalization error. Its proof, analogous to the one of Lemma \ref{lemma:ob-avg-gen}, can be found in Appendix \ref{app:lem-sup}.

In the rest of this section, we provide bounds controlling the worst-case
generalization error for convex, non-convex and strongly convex loss functions.

\subsection{Convex loss functions}

\begin{theorem}\label{thme:worst-convex}
    Assume that the loss function $\ell(\cdot;z)$ is convex, $L$-Lipschitz 
    (Assumption \ref{ass:lipschitz}) and $\beta$-smooth (Assumption \ref{ass:smooth}). Let $A_1(S),\ldots,A_m(S)$ be the $m$ final iterates of D-SGD run for $T$ iterations, with communication graph $W$ satisfying Assumption \ref{ass:doubly} and with $\eta_t\leq 2/\beta$. Then, D-SGD has a bounded worst-case expected generalization error:
    \begin{equation}
        \label{eq:worst-convex}
        \supj|\EE_{A,S}[R(A_j(S)) - R_S(A_j(S))]| \leq 
        \frac{2L^2 \sum_{t=0}^{T-1}\eta_t}{mn}\times \sum_{j=1}^m\supk W_{kj}\;.
    \end{equation}
    %where ${\|W\|}_\infty = \sum_{j=1}^m\sup_k W_{kj}$ is the $\ell_\infty$ operator norm.
\end{theorem}

\begin{proof}[Sketch of proof (see Appendix \ref{app:sup-convex} for details)] 

The proof is analogous to the one obtained for the averaged model (Theorem \ref{thme:convex}). The main difference resides in the fact that we now control $\dsup_{t+1} \triangleq \sup_{k=1,\ldots, m} {\|\theta_k^{(t+1)}  - \Ttheta_k^{(t+1)} \|}_2$ instead of $\dbar_{t+1}=\frac{1}{m}\sum_{k=1}^m {\|\theta_k^{(t+1)}  - \Ttheta_k^{(t+1)} \|}_2$. Let $(i,j)$ denote the $i$-th sample of agent $j$ that has been replaced by another one drawn from the same distribution. Our goal is then equivalent to show that $\EE[\dsup_{T}]\leq \frac{2L\sum_t \eta_t}{n}\sup_k W_{kj}$. Indeed, in that case it suffices to sum this quantity over $i$ and $j$ and divide it by $mn$ to show that D-SGD is worst-model $\varepsilon$-stable (Def. \ref{def:worst-stable}) with $\varepsilon = \frac{2L^2 \sum_{t=0}^{T-1}\eta_t}{mn}\sum_{j=1}^m\sup_k W_{kj}$. A direct use of Lemma \ref{lemma:ob-sup-gen} will conclude the proof.

Again, the analysis is split over two probabilistic events. With probability $1-\frac{1}{n}$, the swapped sample $(i,j)$ is not selected by agent $j$, and it can be proved using tools from Theorem \ref{thme:convex} that $\dsup_{t+1}\leq \dsup_{t}$. 

With probability $\frac{1}{n}$ however, sample $(i,j)$ is selected and in that case we show that $\dsup_{t+1}\leq \dsup_{t} + 2L\eta_t \sup_k{W_{kj}}$. 

In the end we have $\EE[\dsup_T]\leq \EE[\dsup_{T-1}] + \frac{2L \eta_{T-1}}{n}\sup_k W_{kj}$ which can be unraveled until $\dsup_0=0$ to obtain the desired result.
\end{proof}

In contrast to the results of Section~\ref{sec:on-svg}, the bound 
\eqref{eq:worst-convex}
shows that the worst-case generalization error over local
models is impacted by the communication
graph. As expected, we observe that when the graph is complete with uniform
weights $1/m$ (global averaging at each step), we recover the exact same
generalization bound as the one of Theorem~\ref{thme:convex}. On the other
hand, when we take $W$ to be the identity matrix (no interaction between the
agents), the bound becomes $2L^2 \sum_{t=0}^{T-1}\eta_t/n$, which corresponds
to the one obtained by~\citet{hardt2016train} for centralized SGD run over a
dataset of size $n$. %\looseness = -1

The quantity $m^{-1}\sum_{j=1}^m\supk W_{kj}$ measures the connectivity of the
graph $W$. We can relate it to the classical notion of \emph{spectral
gap}, which appears in most of the optimization error bounds 
\citep{lian2017can, ying2021exponential}. Recall that the spectral gap $\rho \in [0,1]$
of a doubly stochastic matrix $W$ is $\rho=1-|\lambda_2(W)|$, $\lambda_2$
being the second-largest eigenvalue of $W$ in module. The following corollary
gives a slightly looser bound that explicitly depends on $\rho$.
\begin{corollary}
    \label{coro:worst-convex}
    Under the conditions of Theorem \ref{thme:worst-convex}, we also have:
    \begin{equation}
        \label{eq:coro-worst-convex}
        \supj|\EE_{A,S}[R(A_j(S)) - R_S(A_j(S))]| \leq
        \Big(\frac{1}{mn} + \frac{1-\rho}{n}\Big)2L^2 \sum_{t=0}^{T-1}\eta_t\;.
    \end{equation}

\end{corollary}

\begin{proof}
    Let $\TW = W - \frac{\1\1^T}{m}$ with $\1$ the unit vector of size $m$. Recall that the largest eigenvalue value $\lambda_1(W)$ of $W$ is equal to $1$ in module and is associated to the eigenvector $\frac{1}{\sqrt{m}}\1$. Hence, the largest eigenvalue of $\TW$ in module is equal to $\lambda_1(\TW)=\lambda_2(W)$. 

    We first notice that $\sum_{j=1}^m\sup_k W_{kj}\leq m {\|W\|}_{\max}$ with ${\|W\|}_{\max}=\sup_{kj}\{W_{kj}\}$ the max norm. Then, a simple use of triangular inequality and matrix norm equivalence gives:
    \begin{align*}
        {\|W\|}_{\max} = {\Big\|\TW + \frac{\1\1^T}{m}\Big\|}_{\max} \leq {\Big\|\frac{\1\1^T}{m}\Big\|}_{\max} + {\|\TW\|}_{\max}  \leq \frac{1}{m} +{\|\TW\|}_2 = \frac{1}m{} + \lambda_2(W)
    \end{align*}

    % To prove the corollary, we need to find an appropriate bound over $\sup_k W_{kj}$. Denote by $e_j$, the $j$-th element of the canonical basis of $\RR^m$, we have:
    % \begin{align*}
    %     \sup_k W_{kj} =  \sup_k \Big|W_{kj} - \frac{1}{m} + \frac{1}{m}\Big| & \leq \frac{1}{m} +  \sup_k \Big|W_{kj} - \frac{1}{m}\Big| = \frac{1}{m} + {\|\TW e_j\|}_\infty = \frac{1}{m} + \frac{{\|\TW e_j\|}_2}{{\|e_j\|}_2 } \\
    %     & \leq \frac{1}{m} + {\|\TW\|}_2 = \frac{1}{m} + 1 - \rho 
    % \end{align*}

    By definition of $\rho$ we can conclude that $\sum_{j=1}^m\sup_k W_{kj}\leq 1 + m(1-\rho)$. Plugging this result into Equation \eqref{eq:worst-convex} finishes the proof.
\end{proof}

%Conclusions regarding this corollary are the same as for Theorem \ref{thme:worst-convex}. 
%The proof of Corollary 
%\ref{coro:worst-convex} is deferred to Appendix \ref{app:sup-convex}.
Again, when $W$ is the complete graph with uniform weights, we have $\rho = 1$ and we
recover the
result of Theorem~\ref{thme:convex}. On the other hand, when $W$ is the
identity matrix, $\rho = 0$ and we recover the rate $\calO(\sum_{t=0}^
{T-1}\eta_t/n)$ of centralized SGD run over $n$ samples.
% This last observation
% was actually expected because in that case, D-SGD is equivalent to SGD run
% independently by the agents over their local data set.
Importantly, the
theorem shows that even in the ``worst-case'' setting, the bound does not
become vacuous for non-connected communication graphs.

% \bat{
% \begin{remark}
%     With $\rho<1$, the bounds are not anymore tending to $0$ as $m$ grows. Its even worst. Could we imagine a better quantity than the spectral gap based on  e.g. Hendricx ?
% \end{remark}
% }


\subsection{Strongly-convex loss functions}


\begin{theorem}\label{thme:worst-strongly}
    Assume that the loss function $\ell(\cdot;z)$ is $\mu$-strongly convex,
    $L$-Lipschitz over $\Theta$ (Assumption~\ref{ass:lipschitz}) and
    $\beta$-smooth (Assumption~\ref{ass:smooth}). Let $A_1(S),\ldots,A_m(S)$
    be the $m$ final iterates of D-SGD run for $T$ iterations, with
    communication graph $W$ satisfying Assumption~\ref{ass:doubly} and with constant stepsize $\eta\leq 1/\beta$. Then, (projected) D-SGD has a bounded worst-case expected generalization error:
    \begin{equation}
        \label{eq:worst-strongly}
        \supj|\EE_{A,S}[R(A_j(S)) - R_S(A_j(S))]| \leq 
        \frac{4L^2 }{\mu mn}\times \sum_{j=1}^m\supk W_{kj}\;.
    \end{equation}
\end{theorem}

The proof of Theorem \ref{thme:worst-strongly} can be found in Appendix \ref{app:sup-strongly}. The same way we proved Corollary \ref{coro:worst-convex}, we can obtain a looser bound involving the spectral gap $\rho$ of $W$, of order $\calO\Big( \frac{1}{ mn}+\frac{1-\rho}{n}\Big)$. Like for the convex case, the more (uniformly) connected is the graph, the closer to $1$ is $\rho$ and the better is the generalization bound, tending towards the one obtained in Theorem \ref{thme:strongly}. Contrary to what can be found in the literature \cite{sun2021stability,taheri2023generalization}, the bound is tending to $0$ as $n$ increases and is not overly impacted by poorly connected graphs.
 


\subsection{Non-convex loss functions}


\begin{theorem}\label{thme:worst-non-convex}
    Assume that $\ell(\cdot;z) \in [0,1]$ is an $L$-Lipschitz
    (Assumption~\ref{ass:lipschitz}) and $\beta$-smooth
    (Assumption~\ref{ass:smooth}) loss
    function for every $z$. Let $A_1(S),\ldots,A_m(S)$ be the $m$ final
    iterates of D-SGD run for $T$ iterations, with communication graph $W$ satisfying Assumption~\ref{ass:doubly} and with monotonically non-increasing step sizes $\eta_t\leq \frac{c}{t+1}$, $c>0$. Then, D-SGD has a bounded worst-case expected generalization error:
    \begin{equation}
        \label{eq:worst-non-convex}
        \supj|\EE_{A,S}[R(A_j(S)) - R_S(A_j(S))]| \leq 
        \tilde{C}\cdot\frac{T^{\frac{\beta c}{\beta c +1}}}{n} \times {\|W\|}_{\max}^{\frac{1}{\beta c +1}}\;,
    \end{equation}
    where ${\|W\|}_{\max}=\sup_{kj}\{W_{kj}\}$ is the max norm and $\tilde{C} =  (1+\frac{1}{\beta c})(2cL^2)^{\frac{1}{\beta c +1}}$.
\end{theorem}

The proof of Theorem \ref{thme:worst-non-convex} is detailed in Appendix \ref{app:sup-non-convex}. Based on the proof of Corollary \ref{coro:worst-convex}, we can again obtain a looser bound of order $\calO\Big( \frac{T^a}{n}(\frac{1}{m}+1-\rho)^{1-a}\Big)$ with $a = \frac{\beta c}{\beta c +1} < 1$. We can also recover, in the same way as for the convex cases of the previous sections, the result of Theorem \ref{thme:non-convex} or the bound for centralized SGD with $n$ data points. Finally, we can note that the rate for non-convex functions is slightly more impacted by the choice of graph $W$. Indeed, since ${\|W\|}_{\max}\leq 1$ (Assumption \ref{ass:doubly}) and $1/(\beta c +1) < 1$, we have $m^{-1}\sum_{j=1}^m\supk W_{kj}\leq {\|W\|}_{\max}\leq {\|W\|}_{\max}^{\frac{1}{\beta c +1}}$.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../neurips_2023"
%%% End:

